Non-Perturbative Renormalisation and Running of BSM Four-Quark Operators in $N_f = 2$ QCD

We perform a non-perturbative study of the scale-dependent renormalisation factors of a complete set of dimension-six four-fermion operators. The renormalisation-group (RG) running is determined in the continuum limit for a specific Schr\"dinger Functional (SF) renormalisation scheme in the framework of lattice QCD with two dynamical flavours ( $N_f = 2$ ). The theory is regularised on a lattice with a plaquette Wilson action and $\mathcal{O}(a)$-improved Wilson fermions. For one of these operators, the computation had been performed in ref. [1]; the present work completes the study for the rest of the operator basis, on the same simulations (configuration ensembles). The related weak matrix elements arise in several operator product expansions; in $\Delta F = 2$ transitions they contain the QCD long-distance effects, including contributions from beyond-Standard Model (BSM) processes. Some of these operators mix under renormalisation and their RG-running is governed by anomalous dimension matrices. In ref. [2] the RG formalism for the operator basis has been worked out in full generality and the anomalous dimension matrix has been calculated in NLO perturbation theory. Here the discussion is extended to the matrix step-scaling functions (matrix-SSFs), which are used in finite-size recursive techniques. We rely on these matrix-SSFs to obtain non-perturbative estimates of the operator anomalous dimensions for scales ranging from $\mathcal{O}(\Lambda_{\rm QCD})$ to $\mathcal{O}(M_W)$.

==> rgi.tex <==
\section{Renormalisation group invariants}
\label{sec:rgi}

In order to obtain a solution of~\req{eq:rg_op} in closed form, it is convenient to
introduce the renormalisation group evolution matrix $U(\mu_2,\mu_1)$
that evolves renormalised operators between scales\footnote{Restricting the evolution operator
to run towards the IR avoids unessential algebraic technicalities below. The running towards
the UV can be trivially obtained by taking $\left[U(\mu_2,\mu_1)\right]^{-1}$.}
$\mu_1$ and $\mu_2<\mu_1$:
\begin{gather}
\label{eq:evol}
\obar{\cQ}_i(\mu_2) = U_{ij}(\mu_2,\mu_1) \obar{\cQ}_j(\mu_1)\,.
\end{gather}
In the rest of this subsection, in order to simplify notation, we will drop the superscripts $\pm$
from quantities $\cQ^\pm, \gamma_{ij}^\pm, U^\pm_{ij}(\mu_2,\mu_1), W^\pm(\mu)$ etc.
Substituting the above into~\req{eq:rg_op} we obtain for the running of $U(\mu_2,\mu_1)$
\begin{gather}
\label{eq:rg_evol}
\mu_2\,\frac{\textcolor{red}{d}}{\textcolor{red}{d}\mu_2}\,U(\mu_2,\mu_1) = \gamma[\gbar(\mu_2)]U(\mu_2,\mu_1)\,,
\end{gather}
with initial condition $U(\mu_1,\mu_1)=\mathbf{1}$. Note that the r.h.s. is a matrix product.
Following a standard procedure, the above expression can be converted into a Volterra-type integral
equation and solved iteratively, viz.
\begin{gather}
U(\mu_2,\mu_1) = \texp\left\{
\int_{\gbar(\mu_1)}^{\gbar(\mu_2)}\kern-8pt\dif g\,\frac{1}{\beta(g)}\,\gamma(g)
\right\}\,,
\label{eq:text-closed}
\end{gather}
where as usual the notation $\texp$ denotes a Taylor expansion of the exponent, in which
each term is an ordered (here $g$-ordered) product. Explicitly, for a generic matrix function $M(x)$, we have
\begin{gather}
\label{eq:texp}
\begin{split}
\texp\left\{\int_{x_-}^{x_+}\kern-8pt\dif x\,M(x)\right\} \equiv \mathbf{1}
&+ \int_{x_-}^{x_+}\kern-8pt\dif x\,M(x) \\
&+ \int_{x_-}^{x_+}\kern-8pt\dif x_1\,M(x_1)\int_{x_-}^{x_1}\kern-8pt\dif x_2\,M(x_2)\\
&+ \int_{x_-}^{x_+}\kern-8pt\dif x_1\,M(x_1)\int_{x_-}^{x_1}\kern-8pt\dif x_2\,M(x_2)\int_{x_-}^{x_2}\kern-8pt\dif x_3\,M(x_3)\\
&+ \ldots\\
= \mathbf{1}
&+ \int_{x_-}^{x_+}\kern-8pt\dif x\,M(x) \\
&+ \frac{1}{2!}\int_{x_-}^{x_+}\kern-8pt\dif x_1\int_{x_-}^{x_+}\kern-8pt\dif x_2\,\Big\{\theta(x_1-x_2)M(x_1)M(x_2)+\\
&~~~~~~~~~~~~~~~~~~~~~~~~~~~~~\theta(x_2-x_1)M(x_2)M(x_1)\Big\}\\
&+ \ldots
\end{split}
\end{gather}
In the specific case of interest, $M(g) = \gamma(g)/\beta(g)$, with $\gamma(g)$ a matrix function and $\beta (g)$ a real function.
To leading order (LO) we have that $M(g) = \gamma^{(0)}/(b_0 g)$ and the independence of the matrix $\gamma^{(0)}$ from the coupling $g$
simplifies eq.~(\ref{eq:texp}), so that the $\texp$ becomes a standard exponential.
One can then easily integrate the exponent in eq.~(\ref{eq:text-closed}) and obtain the LO approximation of the evolution matrix:
\begin{gather}
U(\mu_2,\mu_1) \underset{\rm LO}{=} \left[\frac{\gbar^2(\mu_2)}{\gbar^2(\mu_1)}\right]^{\frac{\gamma^{(0)}}{2b_0}}
\equiv U_{\rm LO}(\mu_2,\mu_1)\,.
\end{gather}
When next-to-leading order corrections are included, the T-exponential becomes non-trivial.
Further insight is gained upon realising that the associativity property of the evolution matrix
$U(\mu_3,\mu_1) = U(\mu_3,\mu_2) U(\mu_2,\mu_1)$ implies that it can actually be factorised
in full generality as
\begin{gather}
\label{eq:fact_U}
U(\mu_2,\mu_1) = \left[\tilde U(\mu_2)\right]^{-1} \tilde U(\mu_1)\,,
\end{gather}
and the matrix  $\tilde U(\mu)$ can be expressed in terms of a matrix $W(\mu)$,
defined through
\begin{gather}
\tilde U(\mu) \equiv \left[\frac{\gbar^2(\mu)}{4\pi}\right]^{-\frac{\gamma^{(0)}}{2b_0}}W(\mu) \,\, .
\end{gather}
The matrix $W$ can be interpreted as the piece of the evolution operator
containing contributions beyond the leading perturbative order.
Putting everything together, we see that
\begin{gather}
\label{eq:def_W}
U(\mu_2,\mu_1) \equiv \left[W(\mu_2)\right]^{-1}\, U_{\rm LO}(\mu_2,\mu_1) W(\mu_1)\,,
\end{gather}
and thus we make contact with the literature (see e.g.~\cite{Buras:2000if,Ciuchini:1997bw}).

Upon inserting~\req{eq:def_W} in~\req{eq:rg_evol} we obtain for $W$ the RG equation
\begin{gather}
\label{eq:rg_W}
\begin{split}
\mu\frac{\textcolor{red}{d}}{\textcolor{red}{d}\mu}W(\mu) &= -W(\mu)\gamma(\gbar(\mu))+\beta(\gbar(\mu))\frac{\gamma^{(0)}}{b_0\gbar(\mu)}W(\mu) \\
&= [\gamma(\gbar(\mu)),W(\mu)] - \beta(\gbar(\mu))\left(
\frac{\gamma(\gbar(\mu))}{\beta(\gbar(\mu))}-\frac{\gamma^{(0)}}{b_0\gbar(\mu)}
\right)W(\mu)\,.
\end{split}
\end{gather}
Expanding perturbatively  we can check~\cite{Papinutto:2016xpq}
that $W$ is regular in the UV, and all the logarithmic divergences
in the evolution operator are contained in $U_{\rm LO}$; in particular,
\begin{gather}
W(\mu)\underset{\mu\to \infty}{=}\mathbf{1}\,.
\end{gather}
%Note also that in the absence of mixing~\req{eq:rg_W} can be solved
%explicitly to get (using $W(0)=1$)
%\begin{gather}
%\label{eq:W_nomix}
%W(\mu)\underset{\rm no~mixing}{=}\exp\left\{
%-\int_{0}^{\gbar(\mu)}\kern-8pt\dif g\,\left[
%\frac{\gamma(g)}{\beta(g)}-\frac{\gamma^{(0)}}{b_0g}
%\right]
%\right\}\,.
%\end{gather}
Rewriting~\req{eq:evol} as
\begin{gather}
\left[\frac{\gbar^2(\mu_2)}{4\pi}\right]^{-\frac{\gamma^{(0)}}{2b_0}}W(\mu_2)\obar{\cQ}(\mu_2)
= \left[\frac{\gbar^2(\mu_1)}{4\pi}\right]^{-\frac{\gamma^{(0)}}{2b_0}}W(\mu_1)\obar{\cQ}(\mu_1)\,.
\end{gather}
and observing that the l.h.s. (respectively r.h.s.) is obviously finite for $\mu_1\to\infty$ (respectively $\mu_2\to\infty$),
we conclude that the vector RGI operators can be obtained as
\begin{gather}
\label{eq:rgi_mix}
\orgi{\cQ} = \left[\frac{\gbar^2(\mu)}{4\pi}\right]^{-\frac{\gamma^{(0)}}{2b_0}}W(\mu)\obar{\cQ}(\mu)\,.
\end{gather}
%When there is no mixing, the use of~\req{eq:W_nomix} immediately brings back~\req{eq:rgi_nomix}.


%\subsection{Perturbative expansion}

%For practical purposes, we will not need a formal solution to~\req{eq:rg_W} that allows to build
%$W$ non-perturbatively. In order to match RGI operators to a hadronic scale, we will actually use the formula
%\begin{gather}
%\label{eq:rgi_practice}
%\orgi{O} = \left[\frac{\gbar^2(\mu_{\rm pt})}{4\pi}\right]^{-\frac{\gamma^{(0)}}{2b_0}}\,W(\mu_{\rm pt})
%\left[U(\mu_{\rm had},\mu_{\rm pt})\right]^{-1}\obar{O}(\mu_{\rm had})\,,
%\end{gather}
%where the evolution $U(\mu_{\rm had},\mu_{\rm pt})$ is constructed non-perturbatively using~\req{eq:evol}
%and the step-scaling functions that will be introduced below,
%and the rest of the expression involves a perturbative matching to the RGI by applying
%\req{eq:rgi_mix} at $\mu=\mu_{\rm pt}$. Thus, all we need is to know about $W$ is its perturbative expansion.

%By expanding~\req{eq:rg_W} perturbatively as
%\begin{gather}
%\label{eq:Wpert}
%W(\mu) \approx \mathbf{1} + \gbar^2(\mu)J(\mu) + \ldots
%\end{gather}
%we find from the $\gbar^2$ and $\gbar^4$ orders the conditions
%\begin{align}
%\frac{\partial}{\partial\mu}J &= 0\,,\\
%\label{eq:J}
%J-\left[\frac{\gamma^{(0)}}{2b_0},J\right] &= \frac{b_1}{2b_0^2}\gamma^{(0)}-\frac{1}{2b_0}\gamma^{(1)}\,,
%\end{align}
%which, modulo sign conventions and the dependence on gauge fixing (which does
%not apply to our context), coincide with Eq.~(24) of~\cite{Ciuchini:1997bw}.
%\req{eq:J} can be easily solved to obtain $J$ for given values of $\gamma^{(0)}$ and $\gamma^{(1)}$.
%The LO and NLO matchings for the RGI thus read
%\begin{align}
%\orgi{O} &\underset{\mbox{\tiny ~\,LO}}{=} \left[\frac{\gbar^2(\mu_{\rm pt})}{4\pi}\right]^{-\frac{\gamma^{(0)}}{2b_0}}\obar{O}(\mu_{\rm pt})\,,\\
%\orgi{O} &\underset{\mbox{\tiny NLO}}{=} \left[\frac{\gbar^2(\mu_{\rm pt})}{4\pi}\right]^{-\frac{\gamma^{(0)}}{2b_0}}\left[\mathbf{1} + %\gbar^2(\mu_{\rm pt})J \right]\obar{O}(\mu_{\rm pt})\,.
%\label{eq:rgi}
%\end{align}









